View Consistency Aware Holistic Triangulation for 3D Human Pose Estimation

The rapid development of multi-view 3D human pose estimation (HPE) is attributed to the maturation of monocular 2D HPE and the geometry of 3D reconstruction. However, 2D detection outliers in occluded views due to neglect of view consistency, and 3D implausible poses due to lack of pose coherence, remain challenges. To solve this, we introduce a Multi-View Fusion module to refine 2D results by establishing view correlations. Then, Holistic Triangulation is proposed to infer the whole pose as an entirety, and anatomy prior is injected to maintain the pose coherence and improve the plausibility. Anatomy prior is extracted by PCA whose input is skeletal structure features, which can factor out global context and joint-by-joint relationship from abstract to concrete. Benefiting from the closed-form solution, the whole framework is trained end-to-end. Our method outperforms the state of the art in both precision and plausibility which is assessed by a new metric.

==> experiment/eq_r_ja.tex <==
\begin{equation}
R_{ja}{(\theta,\varphi)} = \left\{
\begin{array}{lll}
    &1, \quad &(\theta,\varphi)\subset\mathbb{OC} \\
    &0, \quad &others
\end{array}\right.
\label{eq:exp_r_ja}
\end{equation}
% where $\mathbb{OC}$ is the set of all coordinates $(\theta, \varphi)$ whose $OC(\theta, \varphi)=1$.

==> experiment/tb_compare_with_sota.tex <==
\setlength{\tabcolsep}{1pt}
\definecolor{mygray}{gray}{.9}
\begin{table}[t]
\begin{minipage}[t]{0.45\linewidth}
\begin{center}
    \caption{Comparison of MPJPE, inference time and computation complexity on Human3.6M. MACs and param are shorthand of the number of multiply-add operations and parameters which are calculated by thop.}
\label{tb:exp_computation_complexity}
\vspace{-0.7em}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Complexity} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MPJPE\\ (mm)\end{tabular}}  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Time\\ (ms)\end{tabular}}\\ 
% \cline{2-3}
                  & param           & MACs          &                        \\ \midrule
AT\cite{iskakov2019learnable}     & 79M             & 418B          & 19.2   &\textbf{66}                 \\
VT\cite{iskakov2019learnable}    & 80M             & 717B          & \textbf{17.7}          &132         \\ 
\rowcolor{mygray} ours              & \textbf{79M}             & \textbf{418B}          & 19.1  &77                   \\ \bottomrule
\end{tabular}
\end{center}
\end{minipage}
\hspace{1ex}   %%两个minipage之间相隔3个字符的距离
\begin{minipage}[t]{0.55\linewidth}
\begin{center}
    \caption{Comparison with the state of the art on Total Capture in terms of MPJPE. Methods with * are trained on the Total Capture.}
\label{tb:exp_compare_with_sota_tc}
\vspace{-0.7em}
% \setlength{\tabcolsep}{5pt}
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}MPJPE\\ (mm)\end{tabular}} & \multicolumn{3}{c}{Subject1,2,3} & \multicolumn{3}{c}{Subject4,5} & \multirow{2}{*}{Avg.} \\ %\cline{2-7}
                                                                      & W2        & FS3        & A3        & W2       & FS3       & A3        &                      \\ \midrule
% Tri-CPM*\cite{wei2016convolutional}                                                               & 79        & 112        & 106       & 79       & 149       & 73        & 99                   \\
% PVH*\cite{trumble2017total}                                                                   & 48        & 122        & 94        & 84       & 168       & 154       & 107                  \\
% IMUPVH*\cite{trumble2017total}                                                               & 30        & 91         & 49        & 36       & 112       & \textbf{10}        & 70                   \\
AutoEnc*\cite{trumble2018deep}                                                              & \textbf{13}      & 49         & 24        & \textbf{22}      & 71        & 40        & 35                   \\
CrossView*\cite{qiu2019cross}                                                            & 19        & 28         & 21        & 32       & 54       & 33        & 29                  \\ 
GeoFuse*\cite{zhang2020fusing}                                                            & 14        & 26         & 18       & 24       & 49        & \textbf{28}        & 25                   \\ 
\rowcolor{mygray} ours-baseline                                                                  & 64        & 60         & 53        & 72       & 78        & 62        & 63   \\
\rowcolor{mygray} ours-HT                                                                  & 45        & 49         & 45       & 52       & 64       & 57       & 51   \\
\rowcolor{mygray} ours-HT*                                                                  & \textbf{13}        & \textbf{24}         & \textbf{17}        & 23       & \textbf{41}        & 29        & \textbf{23} 
\\ \bottomrule
\end{tabular}
\end{center}
\end{minipage}
\vspace{-1em}
\end{table}
\setlength{\tabcolsep}{1.4pt}
% \footnotetext[1]{https://github.com/Lyken17/pytorch-OpCounter}

==> experiment/tb_matching_strategy.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[t]{\linewidth}
\begin{center}
\caption{\textbf{Effect of matching strategy in MVF.} First row is baseline.}
\label{tb:exp_matching_strategy}
% \vspace{-0.5em}
\resizebox{0.35\textwidth}{!}{
\begin{tabular}{cc|cc|c}
\Xhline{0.09em}
\multicolumn{2}{c|}{Matching Strategy} & \multicolumn{2}{c|}{View} & \begin{tabular}[c]{@{}c@{}}MPJPE\\ (mm)\end{tabular} \\ \cline{1-4}
dot                & fcl               & most-conf    & all   &       \\ \hline
                  &                   &                 &       & 22.60  \\ \hline
    \checkmark               &                   &  \checkmark                   &     & 22.05  \\
      \checkmark                 &               &                   &  \checkmark         & 21.88  \\ \hline
                   &  \checkmark                     &    \checkmark                   &       & 21.92  \\
                   &   \checkmark                    &                   &   \checkmark        & \textbf{21.61}  \\ \Xhline{0.09em}
\end{tabular}}
\end{center}
\vspace{-1.8em}
\end{table}

==> experiment/tb_prior_coefficient_and_feature_extraction.tex <==
\begin{table}[t]
\begin{minipage}[t]{0.5\linewidth}
\begin{center}
\caption{Reconstruction term coefficient comparison. The magnitude of $\lambda$ is $10^3$, and the units of MPJPE-re and PRP@$0.2$ are mm, $\%$ respectively.}
\label{tb:exp_coefficient_pca}
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{l|ccccc}
\Xhline{0.09em}
Coefficient $\lambda$                                            & 1     & 2     & 3     & 4     & 5     \\ \Xhline{0.05em}
MPJPE-re & 22.11 & 22.09 & 22.07 & 22.06 & 22.05 \\
PRP@0.2  & 79.68 & 79.68 & 80.19 & 80.55 & 80.60 \\ \Xhline{0.09em}
Coefficient $\lambda$                                  & 6     & 7     & \textbf{8}     & 9     & 10    \\ \Xhline{0.05em}
MPJPE-re & 22.04 & 22.04 & \textbf{22.04} & 22.05 & 22.06 \\
PRP@0.2 & 80.55 & 80.74 & \textbf{80.97} & 81.02 & 80.74 \\ \Xhline{0.09em}
\end{tabular}
\end{center}
\end{minipage}
\hspace{1ex}   %%两个minipage之间相隔3个字符的距离
\begin{minipage}[t]{0.5\linewidth}
\begin{center}
\caption{Effect of skeletal structural feature strategies. First row is baseline.}
\label{tb:exp_structure_strategy}
\begin{tabular}{ccc|c|c}
\Xhline{0.09em}
\multicolumn{3}{c|}{Strategy} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MPJPE-re\\ (mm)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}PRP$@0.2$\\ (\%)\end{tabular}} \\ \cline{1-3}
dis=0    & dis=1    & dis=2   &                                &                                 \\ \hline
         &          &         & 22.60                          & 79.36                           \\ 
\checkmark        &          &         & 22.04                          & 80.97                           \\
         & \checkmark        &         & 21.86                          & 80.92                           \\
         &          & \checkmark       & 21.91                          & 80.79                           \\ \hline
\checkmark        & \checkmark        &         & 21.83                          & 80.97                           \\
\checkmark        & \checkmark        & \checkmark       & \textbf{21.78}                          & \textbf{81.24}                           \\ \Xhline{0.09em}
\end{tabular}
\end{center}
\end{minipage}
\end{table}


==> method/eq_holistic_triangualtion_with_kcs_closure_answer.tex <==
\begin{gather}
    (A^{T}A+\lambda N^{T}N)Y = \lambda N^{T}N(Y_{root}+Y_{mean})-A^{T}B \nonumber \\ 
    Y =(A^{T}A+\lambda N^{T}N)^{-1} [\lambda N^{T}N(Y_{root}+Y_{mean})-A^{T}B]
\label{eq:method_holistic_triangulation_with_kcs_closure_answer}
\end{gather}

==> method/eq_holistic_triangulation_with_kcs.tex <==
\begin{equation}
    \min\limits_{Y} \quad  \Vert A Y + B\Vert + \lambda \Vert G (V - V^{'}) \Vert
\label{eq:method_holistic_triangulation_with_kcs_0}
\end{equation}
% replace $V$ with Eq.\ref{eq:method_kcs}, the target function can be rewritten as:
% \begin{equation}
%     \min\limits_{Y} \quad  \Vert A Y + B\Vert + \lambda \Vert G (CY - (M^{T}M(CY-CY_{mean})+CY_{mean}) \Vert
% \label{eq:method_holistic_triangulation_with_kcs_1}
% \end{equation}
% where $CY_{mean}$ is the average vector of training data in PCA.

==> method/eq_kinematic_chain_space.tex <==
\vspace{-0.1em}
\begin{gather}
V = CY, \quad Y = GV
\label{eq:method_kcs}
\end{gather}
where $C
% =[\mathbf{c}_{1},\mathbf{c}_{2},\cdots,\mathbf{c}_{J}] 
\in \mathbb{R}^{(3J,3K)}$ is the matrix mapping $Y$ to $V$; $G \in \mathbb{R}^{(3K,3J)}$ maps $V$ back to $Y$ (details in supplementary).
% change to supplementary
% ; and
% \begin{equation}
% \mathbf{c}_j=
% \left[ \begin{array}{@{}*{11}{c}@{}}
% 0 &\cdots &1 &0 &0 &\cdots &-1 &0 &0 &\cdots &0 \\
% 0 &\cdots &0 &1 &0 &\cdots &0 &-1 &0 &\cdots &0 \\
% 0 &\cdots &0 &0 &1 &\cdots &0 &0 &-1 &\cdots &0
% \end{array} \right]
% \label{eq:method_kcs_detail}
% \end{equation}
% which can transform two keypoints with index $i,j$ to the connected bone vector by $\mathbf{y}_{i}-\mathbf{y}_{j}$.

==> method/eq_learnable_triangulation.tex <==
\begin{equation}
    \min \limits_{\mathbf{y}_k} \quad \Vert (\mathbf{w}_k\circ A_k)\mathbf{y}_k + (\mathbf{w}_k\circ \mathbf{b}_k) \Vert
\label{eq:method_learnable_trinagulation}
\end{equation}
where $\mathbf{w}_k=[\omega_{1,k}, \omega_{1,k}, \cdots, \omega_{C,K}, \omega_{C,K}]^{T}$, $\omega_{c,k}$ is the confidence of the $k^{th}$ keypoint in the $c^{th}$ view. $\circ$ is the Hadamard product.

==> method/eq_linear_triangulation.tex <==
\begin{equation}
    \min \limits_{\mathbf{y}_k} \quad \Vert A_k \mathbf{y}_k + \mathbf{b}_k\Vert
\label{eq:method_linear_trinagulation}
\end{equation}
where $A_k\in\mathbb{R}^{(2C,3)}$ is the first three columns of $\widetilde{A}_k$ and $\mathbf{b}_k\in\mathbb{R}^{(2C,1)}$ is the last column. $\widetilde{A}_k$ is computed by multi-view 2D positions $\mathbf{x}_k$ and the corresponding camera projection matrices $P_c$ (refer to supplementary material for derivation). 
% add Ay=0 in supplementary material

==> method/eq_matching_heatmap.tex <==
\begin{equation}
    H_{match}(i,j) = sim ( F(i,j), F(p^{'}) )
\label{eq:method_matching_heatmap}
\end{equation}
where $F$ represents the features generated by 2D backbone, $F(p^{'})$ is the sampled feature according to the location $p^{'}$ via bilinear interpolation.

==> method/fig_pca_and_skeletal_structure.tex <==
\begin{figure}[t]

% \begin{minipage}[t]{\linewidth}
%     \centering
%     \includegraphics[width=0.9\textwidth]{method/reconstructionterm.pdf}
%     % \vspace{-1.6em}
%     \caption{Effect of two terms in our HT.}
%     \label{fig:method_pca_reconstruction_term}
% % \end{figure}
% \end{minipage}
% % \vspace{1ex}   %%两个minipage之间相隔3个字符的距离
% \begin{minipage}[t]{\linewidth}
% \begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{method/skeletalstructure.pdf}
    \vspace{-1em}
    \caption{Skeletal structure features.}
    \label{fig:method_skeletal_structure}
% \end{minipage}
\vspace{-1em}
\end{figure}
